Learning Generalizable Locomotion Skills with Hierarchical Reinforcement Learning

Learning to locomote to arbitrary goals on hardware remains a challenging problem for reinforcement learning. In this paper, we present a hierarchical learning framework that improves sample-efficiency and generalizability of locomotion skills on real-world robots. Our approach divides the problem of goal-oriented locomotion into two sub-problems: learning diverse primitives skills, and using model-based planning to sequence these skills. We parametrize our primitives as cyclic movements, improving sample-efficiency of learning on a 18 degrees of freedom robot. Then, we learn coarse dynamics models over primitive cycles and use them in a model predictive control framework. This allows us to learn to walk to arbitrary goals up to 12m away, after about two hours of training from scratch on hardware. Our results on a Daisy hexapod hardware and simulation demonstrate the efficacy of our approach at reaching distant targets, in different environments and with sensory noise.

==> controllers.tex <==
\section{Experimental set up}
%\AR{Either remove this section, or make it just the robot? Can also just make it all part of experiments}


\subsection{Model - Lookup table }
As mentioned in the former section, the high-level control choose the action in an model-based way. Usually, the model in model-based RL is represent by a deep neural network(DNN), since DNN has high capacity to capture all mapping of the dynamics function $s_{t+1}=F(s_t,a_t)$, especially when state and action are continuous. 


However, in our settings, the dynamics of the high-level control is defined as: $\delta s=f_\theta(a_i)$
here $\Delta s$ is the position and orientation change of center of mass in the last time step's center of mass coordinate, $\Delta s = (r, \alpha,\beta)$
%add a plot here
as shown on the plot, the $r, \alpha$ indicates the position variation of the center of mass while $\beta$ shows the robots' orientation change. We also assume that no outside factor will influence the consequence of a certain action. Therefore, the number of possible input of the dynamics model has been shrank into the total amount of elementary motions we have. So we use a lookup table as our dynamics model. Comparing to DNN lookup table has several advantages:
\begin{itemize}

    \item Reusable: comparing to DNN the elements in lookup table is more independent, while different elements share the same neural network. In the future, when we have more elementary motions, we can directly add their dynamics model into the lookup table without affects others, but for DNN we might need to retain the whole network to fit for all actions.
    \item Fast: when using the saved dynamic model to do model-based control lookup table is faster to computing the result since, it can directly search for the result, while DNN needs to go through a neural network to get the prediction.
    
\end{itemize}


